A New Acceleration Paradigm for Discrete CosineTransform and Other Fourier-Related Transforms

Discrete cosine transform (DCT) and other Fourier-related transforms have broad applications in scientific computing. However, off-the-shelf high-performance multi-dimensional DCT (MD DCT) libraries are not readily available in parallel computing systems. Public MD DCT implementations leverage a straightforward method that decomposes the computation into multiple 1D DCTs along every single dimension, which inevitably has non-optimal performance due to low computational efficiency, parallelism, and locality. In this paper, we propose a new acceleration paradigm for MD DCT. A three-stage procedure is proposed to factorize MD DCT into MD FFT and highly-optimized preprocessing/postprocessing with efficient computation and high arithmetic intensity. Our paradigm can be easily extended to other Fourier-related transforms and other parallel computing systems. Experimental results show that our 2D DCT/IDCT CUDA implementation has a stable, FFT-comparable execution time, which is $2\times$ faster than the previous row-column method. Several case studies demonstrate that a promising efficiency improvement can be achieved with our paradigm. The implementations are available at https://github.com/JeremieMelo/dct_cuda/tree/reconstruct.

==> doc/7acknowledgement.tex <==
\section{Acknowledgments}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

This section has a special environment:
\begin{verbatim}
  \begin{acks}
  ...
  \end{acks}
\end{verbatim}
so that the information contained therein can be more easily collected
during the article metadata extraction phase, and to ensure
consistency in the spelling of the section heading.

Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

\section*{Acknowledgements}
This document is derived from two previous conferences, in particular HPCA 2021 and MICRO 2021, which, in turn, are derived from past MICRO, HPCA, ISCA, and ASPLOS conferences.

